Trajectory Generation for Millimeter Scale Ferromagnetic Swimmers: Theory and Experiments

Microrobots have the potential to impact many areas such as microsurgery, micromanipulation and minimally invasive sensing. Due to their small size, microrobots swim in a regime that is governed by low Reynolds number hydrodynamics. In this paper, we consider small scale artificial swimmers that are fabricated using ferromagnetic filaments and locomote in response to time varying external magnetic fields. We motivate the design of previously proposed control laws using tools from geometric mechanics and also demonstrate how new control laws can be synthesized to generate net translation in such swimmers. We further describe how to modify these control inputs to make the swimmers track rich trajectories in the workspace by investigating stability properties of their limit cycles in the orientation angles phase space. Following a systematic design optimization, we develop a principled approach to encode internal magnetization distributions in millimeter scale ferromagnetic filaments. We verify and demonstrate this procedure experimentally and finally show translation, trajectory tracking and turning in place locomotion in these optimal swimmers using a Helmholtz coils setup.

==> References.tex <==
% modular robots

@inproceedings{divelbiss1992global,
  title={A global approach to nonholonomic motion planning},
  author={Divelbiss, AW and Wen, J},
  booktitle={Decision and Control, 1992., Proceedings of the 31st IEEE Conference on},
  pages={1597--1602},
  year={1992},
  organization={IEEE}
}

@article{koiller1996problems,
	title={Problems and progress in microswimming},
	author={Koiller, Jair and Ehlers, Kurt and Montgomery, Richard},
	journal={Journal of Nonlinear Science},
	volume={6},
	number={6},
	pages={507--541},
	year={1996},
	publisher={Springer}
}

@article{sendoh2003fabrication,
	title={Fabrication of magnetic actuator for use in a capsule endoscope},
	author={Sendoh, Masahiko and Ishiyama, Kazushi and Arai, K-I},
	journal={IEEE Transactions on Magnetics},
	volume={39},
	number={5},
	pages={3232--3234},
	year={2003},
	publisher={IEEE}
}

@misc{cole1976perturbation,
	title={Perturbation Methods (Ali Hasan Nayfeh)},
	author={Cole, Julian D},
	year={1976},
	publisher={Society for Industrial and Applied Mathematics}
}

@article{diller2014continuously,
	title={Continuously distributed magnetization profile for millimeter-scale elastomeric undulatory swimming},
	author={Diller, Eric and Zhuang, Jiang and Zhan Lum, Guo and Edwards, Matthew R and Sitti, Metin},
	journal={Applied Physics Letters},
	volume={104},
	number={17},
	pages={174101},
	year={2014},
	publisher={AIP}
}

@article{jang2015undulatory,
	title={Undulatory Locomotion of Magnetic Multilink Nanoswimmers},
	author={Jang, B and Gutman, E and Stucki, N and Seitz, BF and Wendel Garcia, PD and Newton, T and Pokki, J and Ergeneman, O and Pane, S and Or, Y and others},
	journal={Nano letters},
	volume={15},
	number={7},
	pages={4829},
	year={2015}
}

@article{cebers2003dynamics,
	title={Dynamics of a chain of magnetic particles connected with elastic linkers},
	author={Cebers, Andrejs},
	journal={Journal of Physics: Condensed Matter},
	volume={15},
	number={15},
	pages={S1335},
	year={2003},
	publisher={IOP Publishing}
}

@article{cebers2003dynamics,
	title={Dynamics of a chain of magnetic particles connected with elastic linkers},
	author={Cebers, Andrejs},
	journal={Journal of Physics: Condensed Matter},
	volume={15},
	number={15},
	pages={S1335},
	year={2003},
	publisher={IOP Publishing}
}

@article{koenig2005magnetic,
	title={Magnetic force probe for nanoscale biomolecules},
	author={Koenig, A and Hebraud, Pascal and Gosse, C and Dreyfus, R and Baudry, J and Bertrand, E and Bibette, J},
	journal={Physical review letters},
	volume={95},
	number={12},
	pages={128301},
	year={2005},
	publisher={APS}
}

@article{cebers2016flexible,
	title={Flexible magnetic filaments and their applications},
	author={Cebers, Andrejs and Erglis, Kaspars},
	journal={Advanced Functional Materials},
	volume={26},
	number={22},
	pages={3783--3795},
	year={2016},
	publisher={Wiley Online Library}
}


@article{gadelha2013optimal,
	title={On the optimal shape of magnetic swimmers},
	author={Gad{\^e}lha, Hermes},
	journal={Regular and Chaotic Dynamics},
	volume={18},
	number={1-2},
	pages={75--84},
	year={2013},
	publisher={Springer}
}

@inproceedings{bell2007flagella,
	title={Flagella-like propulsion for microrobots using a nanocoil and a rotating electromagnetic field},
	author={Bell, Dominik J and Leutenegger, S and Hammar, KM and Dong, LX and Nelson, Bradley J},
	booktitle={Robotics and Automation, 2007 IEEE International Conference on},
	pages={1128--1133},
	year={2007},
	organization={IEEE}
}

@article{ghosh2009controlled,
	title={Controlled propulsion of artificial magnetic nanostructured propellers},
	author={Ghosh, Ambarish and Fischer, Peer},
	journal={Nano letters},
	volume={9},
	number={6},
	pages={2243--2245},
	year={2009},
	publisher={ACS Publications}
}
@article{belovs2009ferromagnetic,
	title={Ferromagnetic microswimmer},
	author={Belovs, M and C{\=e}bers, A},
	journal={Physical Review E},
	volume={79},
	number={5},
	pages={051503},
	year={2009},
	publisher={APS}
}
@incollection{pak2015theoretical,
	title={Theoretical models of low-Reynolds-number locomotion},
	author={Lauga, Eric},
	booktitle={Fluid-Structure Interactions in Low-Reynolds-Number Flows},
	pages={100--167},
	year={2015},
	publisher={Royal Society of Chemistry}
}


@article{gao2012cargo,
	title={Cargo-towing fuel-free magnetic nanoswimmers for targeted drug delivery},
	author={Gao, Wei and Kagan, Daniel and Pak, On Shun and Clawson, Corbin and Campuzano, Susana and Chuluun-Erdene, Erdembileg and Shipton, Erik and Fullerton, Eric E and Zhang, Liangfang and Lauga, Eric and others},
	journal={small},
	volume={8},
	number={3},
	pages={460--467},
	year={2012},
	publisher={Wiley Online Library}
}

@article{honda1996micro,
	title={Micro swimming mechanisms propelled by external magnetic fields},
	author={Honda, T and Arai, KI and Ishiyama, K},
	journal={IEEE Transactions on Magnetics},
	volume={32},
	number={5},
	pages={5085--5087},
	year={1996},
	publisher={IEEE}
}

@article{alouges2017purcell,
	title={Purcell magneto-elastic swimmer controlled by an external magnetic field},
	author={Alouges, Fran{\c{c}}ois and Desimone, Antonio and Giraldi, Laetitia and Zoppello, Marta},
	journal={IFAC-PapersOnLine},
	volume={50},
	number={1},
	pages={4120--4125},
	year={2017},
	publisher={Elsevier}
}


@article{khalil2014magnetosperm,
	title={MagnetoSperm: A microrobot that navigates using weak magnetic fields},
	author={Khalil, Islam SM and Dijkslag, Herman C and Abelmann, Leon and Misra, Sarthak},
	journal={Applied Physics Letters},
	volume={104},
	number={22},
	pages={223701},
	year={2014},
	publisher={AIP}
}


@article{nelson2010microrobots,
	title={Microrobots for minimally invasive medicine},
	author={Nelson, Bradley J and Kaliakatsos, Ioannis K and Abbott, Jake J},
	journal={Annual review of biomedical engineering},
	volume={12},
	pages={55--85},
	year={2010},
	publisher={Annual Reviews}
}
@article{goyeau2017dynamics,
	title={Dynamics of a flexible ferromagnetic filament in a rotating magnetic field},
	author={Goyeau, L and Livanovi{\v{c}}s, R and C{\=e}bers, A},
	journal={Physical Review E},
	volume={96},
	number={6},
	pages={062612},
	year={2017},
	publisher={APS}
}
@article{peyer2013bio,
	title={Bio-inspired magnetic swimming microrobots for biomedical applications},
	author={Peyer, Kathrin E and Zhang, Li and Nelson, Bradley J},
	journal={Nanoscale},
	volume={5},
	number={4},
	pages={1259--1272},
	year={2013},
	publisher={Royal Society of Chemistry}
}

@article{tam2007optimal,
  title={Optimal stroke patterns for Purcell’s three-link swimmer},
  author={Tam, Daniel and Hosoi, Annete E},
  journal={Physical Review Letters},
  volume={98},
  number={6},
  pages={068105},
  year={2007},
  publisher={APS}
}

@article{shapere1989geometry,
	title={Geometry of self-propulsion at low Reynolds number},
	author={Shapere, Alfred and Wilczek, Frank},
	journal={Journal of Fluid Mechanics},
	volume={198},
	pages={557--585},
	year={1989},
	publisher={Cambridge University Press}
}

@article{wiezel2016optimization,
  title={Optimization and small-amplitude analysis of Purcell's three-link microswimmer model},
  author={Wiezel, Oren and Or, Yizhar},
  journal={arXiv preprint arXiv:1603.02268},
  year={2016}
}


@article{hatton2011geometric,
  title={Geometric motion planning: The local connection, Stokes’ theorem, and the importance of coordinate choice},
  author={Hatton, Ross L and Choset, Howie},
  journal={The International Journal of Robotics Research},
  volume={30},
  number={8},
  pages={988--1014},
  year={2011},
  publisher={SAGE Publications}
}

@inproceedings{hatton2008connection,
  title={Connection vector fields for underactuated systems},
  author={Hatton, Ross L and Choset, Howie},
  booktitle={2008 2nd IEEE RAS \& EMBS International Conference on Biomedical Robotics and Biomechatronics},
  pages={451--456},
  year={2008},
  organization={IEEE}
}

@article{becker2003self,
  title={On self-propulsion of micro-machines at low Reynolds number: Purcell's three-link swimmer},
  author={Becker, Leif E and Koehler, Stephan A and Stone, Howard A},
  journal={Journal of fluid mechanics},
  volume={490},
  pages={15--35},
  year={2003},
  publisher={Cambridge Univ Press}
}

@incollection{ostrowski1996geometric,
  title={Geometric perspectives on the mechanics and control of robotic locomotion},
  author={Ostrowski, Jim and Burdick, Joel},
  booktitle={Robotics Research},
  pages={536--547},
  year={1996},
  publisher={Springer}
}


@article{berg2002spiroplasma,
  title={How Spiroplasma might swim},
  author={Berg, Howard C},
  journal={Journal of bacteriology},
  volume={184},
  number={8},
  pages={2063--2064},
  year={2002},
  publisher={Am Soc Microbiol}
}

@article{purcell1977life,
  title={Life at low Reynolds number},
  author={Purcell, Edward M},
  journal={Am. J. Phys},
  volume={45},
  number={1},
  pages={3--11},
  year={1977}
}


@inproceedings{giraldi2013controllability,
  title={Controllability and optimal strokes for N-link microswimmer},
  author={Giraldi, Laetitia and Martinon, Pierre and Zoppello, Marta},
  booktitle={52nd IEEE Conference on Decision and Control},
  pages={3870--3875},
  year={2013},
  organization={IEEE}
}


@article{avron2008geometric,
  title={A geometric theory of swimming: Purcell's swimmer and its symmetrized cousin},
  author={Avron, JE and Raz, O},
  journal={New Journal of Physics},
  volume={10},
  number={6},
  pages={063016},
  year={2008},
  publisher={IOP Publishing}
}


@inproceedings{lafferriere1991motion,
  title={Motion planning for controllable systems without drift},
  author={Lafferriere, G and Sussmann, H},
  booktitle={Robotics and Automation, 1991. Proceedings., 1991 IEEE International Conference on},
  pages={1148--1153},
  year={1991},
  organization={IEEE}
}


@inproceedings{gong2016simplifying,
	title={Simplifying Gait Design via Shape Basis Optimization.},
	author={Gong, Chaohui and Goldman, Daniel I and Choset, Howie}
}

@article{kelly2011mechanics,
	title={The mechanics and control of driftless swimming},
	author={Kelly, SCOTT DAVID},
	journal={SIAM J. of Control and Optimization},
	year={2011}
}

@article{ostrowski1998geometric,
	title={The geometric mechanics of undulatory robotic locomotion},
	author={Ostrowski, Jim and Burdick, Joel},
	journal={The international journal of robotics research},
	volume={17},
	number={7},
	pages={683--701},
	year={1998},
	publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@book{murray1994mathematical,
	title={A mathematical introduction to robotic manipulation},
	author={Murray, Richard M and Li, Zexiang and Sastry, S Shankar and Sastry, S Shankara},
	year={1994},
	publisher={CRC press}
}

@article{rollinson2012virtual,
	title={Virtual chassis for snake robots: Definition and applications},
	author={Rollinson, David and Buchan, Austin and Choset, Howie},
	journal={Advanced Robotics},
	volume={26},
	number={17},
	pages={2043--2064},
	year={2012},
	publisher={Taylor \& Francis}
}
@article{purcell1989helmholtz,
	title={Helmholtz coils revisited},
	author={Purcell, Edward M},
	journal={American Journal of Physics},
	volume={57},
	number={1},
	pages={18--22},
	year={1989},
	publisher={AAPT}
}
@article{cox1970motion,
	title={The motion of long slender bodies in a viscous fluid part 1. general theory},
	author={Cox, RG},
	journal={Journal of Fluid mechanics},
	volume={44},
	number={4},
	pages={791--810},
	year={1970},
	publisher={Cambridge University Press}
}
@article{hatton2013geometric,
	title={Geometric swimming at low and high Reynolds numbers},
	author={Hatton, Ross L and Choset, Howie},
	journal={IEEE Transactions on Robotics},
	volume={29},
	number={3},
	pages={615--624},
	year={2013},
	publisher={IEEE}
}
@article{roper2006dynamics,
	title={On the dynamics of magnetically driven elastic filaments},
	author={Roper, Marcus and Dreyfus, R{\'e}mi and Baudry, Jean and Fermigier, Marc and Bibette, J{\'e}r{\^o}me and Stone, Howard A},
	journal={Journal of Fluid Mechanics},
	volume={554},
	pages={167--190},
	year={2006},
	publisher={Cambridge University Press}
}
@article{hirose2009snake,
	title={Snake-like robots [tutorial]},
	author={Hirose, Shigeo and Yamada, Hiroya},
	journal={IEEE Robotics \& Automation Magazine},
	volume={16},
	number={1},
	pages={88--98},
	year={2009},
	publisher={IEEE}
}
@article{gadelha2013optimal,
	title={On the optimal shape of magnetic swimmers},
	author={Gad{\^e}lha, Hermes},
	journal={Regular and Chaotic Dynamics},
	volume={18},
	number={1-2},
	pages={75--84},
	year={2013},
	publisher={Springer}
}
@article{gutman2016optimizing,
	title={Optimizing an undulating magnetic microswimmer for cargo towing},
	author={Gutman, Emiliya and Or, Yizhar},
	journal={Physical Review E},
	volume={93},
	number={6},
	pages={063105},
	year={2016},
	publisher={APS}
}


@article{gutman2014simple,
	title={Simple model of a planar undulating magnetic microswimmer},
	author={Gutman, Emiliya and Or, Yizhar},
	journal={Physical Review E},
	volume={90},
	number={1},
	pages={013012},
	year={2014},
	publisher={APS}
}
@article{dreyfus2005microscopic,
	title={Microscopic artificial swimmers},
	author={Dreyfus, R{\'e}mi and Baudry, Jean and Roper, Marcus L and Fermigier, Marc and Stone, Howard A and Bibette, J{\'e}r{\^o}me},
	journal={Nature},
	volume={437},
	number={7060},
	pages={862},
	year={2005},
	publisher={Nature Publishing Group}
}


@article{alouges2015can,
	title={Can magnetic multilayers propel artificial microswimmers mimicking sperm cells?},
	author={Alouges, Fran{\c{c}}ois and DeSimone, Antonio and Giraldi, Laetitia and Zoppello, Marta},
	journal={Soft Robotics},
	volume={2},
	number={3},
	pages={117--128},
	year={2015},
	publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{alouges2017purcell,
	title={Purcell magneto-elastic swimmer controlled by an external magnetic field},
	author={Alouges, Fran{\c{c}}ois and Desimone, Antonio and Giraldi, Laetitia and Zoppello, Marta},
	journal={IFAC-PapersOnLine},
	volume={50},
	number={1},
	pages={4120--4125},
	year={2017},
	publisher={Elsevier}
}

@article{alouges2013self,
	title={Self-propulsion of slender micro-swimmers by curvature control: N-link swimmers},
	author={Alouges, F and DeSimone, Antonio and Giraldi, L and Zoppello, M},
	journal={International Journal of Non-Linear Mechanics},
	volume={56},
	pages={132--141},
	year={2013},
	publisher={Elsevier}
}

@article{cicconofri2016motion,
	title={Motion planning and motility maps for flagellar microswimmers},
	author={Cicconofri, Giancarlo and DeSimone, Antonio},
	journal={The European Physical Journal E},
	volume={39},
	number={7},
	pages={72},
	year={2016},
	publisher={Springer}
}

@article{gutman2016symmetries,
	title={Symmetries and gaits for Purcell's three-link microswimmer model},
	author={Gutman, Emiliya and Or, Yizhar},
	journal={IEEE Transactions on Robotics},
	volume={32},
	number={1},
	pages={53--69},
	year={2016},
	publisher={IEEE}
}

@phdthesis{burton2013dynamics,
	title={The dynamics and kinematics of bio-in swimming systems},
	author={Burton, Lisa Janelle},
	year={2013},
	school={Massachusetts Institute of Technology}
}

@article{murray1993nonholonomic,
	title={Nonholonomic motion planning: Steering using sinusoids},
	author={Murray, Richard M and Sastry, S Shankar},
	journal={IEEE Transactions on Automatic Control},
	volume={38},
	number={5},
	pages={700--716},
	year={1993},
	publisher={IEEE}
}

@article{cho2014mini,
	title={Mini and micro propulsion for medical swimmers},
	author={Cho, Sung Kwon and others},
	journal={Micromachines},
	volume={5},
	number={1},
	pages={97--113},
	year={2014},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@article{nelson2010microrobots,
	title={Microrobots for minimally invasive medicine},
	author={Nelson, Bradley J and Kaliakatsos, Ioannis K and Abbott, Jake J},
	journal={Annual review of biomedical engineering},
	volume={12},
	pages={55--85},
	year={2010},
	publisher={Annual Reviews}
}

@article{kelly1995geometric,
	title={Geometric phases and robotic locomotion},
	author={Kelly, Scott D and Murray, Richard M},
	journal={Journal of Field Robotics},
	volume={12},
	number={6},
	pages={417--431},
	year={1995},
	publisher={Wiley Online Library}
}

@article{hatton2009approximating,
	title={Approximating displacement with the body velocity integral},
	author={Hatton, Ross L and Choset, Howie},
	year={2009}
}

@article{melli2006motion,
	title={Motion planning for an articulated body in a perfect planar fluid},
	author={Melli, Juan B and Rowley, Clarence W and Rufat, Dzhelil S},
	journal={SIAM Journal on applied dynamical systems},
	volume={5},
	number={4},
	pages={650--669},
	year={2006},
	publisher={SIAM}
}
